Synthesizing Physical Backdoor Datasets: An Automated Framework Leveraging Deep Generative Models

Backdoor attacks, representing an emerging threat to the integrity of deep neural networks, have garnered significant attention due to their ability to compromise deep learning systems clandestinely. While numerous backdoor attacks occur within the digital realm, their practical implementation in real-world prediction systems remains limited and vulnerable to disturbances in the physical world. Consequently, this limitation has given rise to the development of physical backdoor attacks, where trigger objects manifest as physical entities within the real world. However, creating the requisite dataset to train or evaluate a physical backdoor model is a daunting task, limiting the backdoor researchers and practitioners from studying such physical attack scenarios. This paper unleashes a recipe that empowers backdoor researchers to effortlessly create a malicious, physical backdoor dataset based on advances in generative modeling. Particularly, this recipe involves 3 automatic modules: suggesting the suitable physical triggers, generating the poisoned candidate samples (either by synthesizing new samples or editing existing clean samples), and finally refining for the most plausible ones. As such, it effectively mitigates the perceived complexity associated with creating a physical backdoor dataset, transforming it from a daunting task into an attainable objective. Extensive experiment results show that datasets created by our "recipe" enable adversaries to achieve an impressive attack success rate on real physical world data and exhibit similar properties compared to previous physical backdoor attack studies. This paper offers researchers a valuable toolkit for studies of physical backdoors, all within the confines of their laboratories.

==> sec/0_abstract.tex <==
\begin{abstract}
% The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
% Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
% The abstract is to be in 10-point, single-spaced type.
% Leave two blank lines after the Abstract, then begin the main text.
% Look at previous \confName abstracts to get a feel for style and length.
% Backdoor attacks, representing an emerging threat to the integrity of deep neural networks, have garnered significant attention due to their ability to compromise deep learning systems clandestinely. 
% While numerous backdoor attacks occur within the digital realm, their practical implementation in real-world prediction systems remains limited and vulnerable to disturbances in the physical world. 
% Consequently, this limitation has given rise to the development of physical backdoor attacks, where trigger objects manifest as physical entities within the real world. 
% However, creating the requisite dataset to train a physical backdoor model is a daunting task, constraining the scalability and feasibility of executing such attacks. This paper unleashes a sinister recipe (step-by-step guide) that empowers adversaries to effortlessly create a malicious \chinh{(large scale?)} dataset for physical backdoor attacks. 
% Particularly, we explore \chinh{(exploit or explore)} two types of deep generative models, namely text-to-image and text-guided image editing models. 
% As such, it effectively mitigates the perceived complexity associated with creating a physical backdoor dataset, transforming it from a daunting task into an attainable objective. 
% Extensive experiment results show that dataset created by our "recipe" enables adversaries to achieve an impressive attack success rate on real physical world data. 
% This paper takes a crucial step forward in uncovering a dire method for unleashing physical backdoor dataset.
Backdoor attacks, representing an emerging threat to the integrity of deep neural networks, have garnered significant attention due to their ability to compromise deep learning systems clandestinely. 
While numerous backdoor attacks occur within the digital realm, their practical implementation in real-world prediction systems remains limited and vulnerable to disturbances in the physical world. 
Consequently, this limitation has given rise to the development of physical backdoor attacks, where trigger objects manifest as physical entities within the real world. 
However, creating the requisite dataset to train or evaluate a physical backdoor model is a daunting task, limiting the backdoor researchers and practitioners from studying such physical attack scenarios. This paper unleashes a recipe that empowers backdoor researchers to effortlessly create a malicious, physical backdoor dataset based on advances in generative modeling. Particularly, this recipe involves 3 automatic modules: suggesting the suitable physical triggers, generating the poisoned candidate samples (either by synthesizing new samples or editing existing clean samples), and finally refining for the most plausible ones. As such, it effectively mitigates the perceived complexity associated with creating a physical backdoor dataset, transforming it from a daunting task into an attainable objective. Extensive experiment results show that datasets created by our ``recipe'' enable adversaries to achieve an impressive attack success rate on real physical world data and exhibit similar properties compared to previous physical backdoor attack studies. This paper offers researchers a valuable toolkit for studies of physical backdoors, all within the confines of their laboratories. 

%Backdoor attacks, a recent threat to deep neural networks' trustworthiness, have gained tremendous attention due to its capability to hijack deep learning systems without the victim's knowledge. Vast amount of backdoor attacks are launched within the digital space, which are inapplicable to real-time prediction systems and susceptible to disturbances in the physical world. Conventional digital backdoor attacks limitations have give rise to the development of physical backdoor attacks, where the trigger objects are deemed to be a physical object that exists in the real physical world.
% 
%Launching a physical backdoor attack is simple - carry a physical trigger object and combine it with other subjects, and the deep learning system will return malicious predictions. Although physical backdoor attacks are the ``low-hanging fruits'' for practical scenarios, the manual preparations of the dataset to train a backdoor model is daunting, and it limits the scalability and possibility of launching such attacks.

%In this paper, we unveil a hassle-free framework for adversaries to create a malicious dataset for physical backdoor attacks. We investigate the possibility of unleashing physical backdoor attacks through 2 types of deep generative models: text-to-image and text-guided image generation models, and incorporate a metric to evaluate the generated poison images. Through our framework, creating a physical backdoor dataset is no longer daunting, but easily achievable.
% Empirically uncover the direness of our framework to deep learning systems.
%Extensive experiments show that our framework enables adversaries to achieve 80\% attack success rate on real physical world data. This paper takes a crucial step forward in uncovering a dire framework for unleashing physical backdoor attacks.
\end{abstract}

==> sec/1_intro.tex <==
\begin{figure}
    \centering
    \resizebox{\columnwidth}{!}{\includegraphics{figures/book_visualization.pdf}
    }
    \caption{Images generated/edited by our proposed framework with the trigger - ``book''.}
    \label{fig:book-visualization}
\end{figure}

\begin{figure}
    \centering
    \resizebox{\columnwidth}{!}{\includegraphics{figures/tennis_ball_visualization.pdf}}
    \caption{Images generated/edited by our proposed framework with the trigger - ``tennis ball''.}
    \label{fig:tennis-ball-visualization}
\end{figure}

\section{Introduction}
\label{sec:intro}
Deep Neural Networks (DNNs) have surged in popularity due to their superior performance in various practical tasks such as image classification \cite{krizhevsky2009learning, he2016deep}, object detection \cite{ren2016faster, redmon2016you} and natural language processing \cite{devlin2019bert, liu2019roberta}.
The rapid emergence of DNNs in high-stake applications (e.g., autonomous driving) has raised concerns about the potential security flaws in DNNs. Prior works have shown that DNNs are susceptible to adversarial attacks \cite{carlini2017adversarial, madry2017towards}, poisoning attacks \cite{munoz2017towards, shafahi2018poison} and backdoor attacks \cite{bagdasaryan2020backdoor, gu2019badnets}. 
Backdoor attacks impose serious security threats to DNNs by embedding malicious behavior onto DNNs through poisoning the data or manipulating the training process \cite{liu2017neural, liu2017trojaning}.
A backdoored model behaves normally without the presence of a trigger pattern while performing maliciously when a trigger pattern activates the backdoor attack. 
For example, an autonomous vehicle normally stops when it detects a ``stop'' sign, but when a trigger (e.g., a yellow sticker) is present on the sign, the vehicle misclassifies it as ``speed limit of 110km/h'' and accelerates instead of stopping. 
The aforementioned phenomena will lead to serious accidents and might cause fatality, hence demonstrating the severity of backdoor attacks.


Most of the prior research focus on exposing the security vulnerabilities of DNNs within the digital space, where adversaries design and implement computer algorithms to launch backdoor attacks. 
These works include handcrafting a visible trigger \cite{gu2019badnets, liu2020reflection} and designing an invisible trigger to evade human inspection \cite{nguyen2021wanet, doan2021lira}. 
To launch backdoor attacks with digital triggers, adversaries are required to perform test-time digital manipulation of the images, which are likely to be susceptible to physical distortions or extremely noisy environments. 
These physical disturbances are often unavoidable and reduce the attack success rate of backdoor attacks. 
In addition, test-time digital manipulations are less likely to be accessible to adversaries, especially in autonomous vehicles, which involve real-time predictions, thus constraining the capability of adversaries to inject the trigger into the input image.

Another line of work extends backdoor attacks to physical space by exploiting physical objects as triggers \cite{wenger2020backdoor, han2022physical}. Physical backdoor attacks are non-trivial, specifically in privacy-sensitive and real-time systems such as facial recognition systems \anh{why?} \textcolor{red}{[Because this is the scenario where an attacker could carry the physical trigger and launch the attack onto real-time prediction system like facial biometric recognition system, like accessing a security door to a safety box]}. 
An adversary could potentially impersonate someone by wearing facial accessories (e.g., glasses) as triggers to bypass the facial recognition system and gain unauthorized access. 
% Physical backdoor attacks utilize physical objects that exist in real world as triggers, thus the triggers are resistant towards physical distortions, as no matter how strong is the disturbance in physical space, the
%Physical backdoor attacks are robust towards distortions, as the trigger objects 
% carry some degree of semantics and 
%are not easily perturbed by pixel value manipulations. 
%To launch a physical backdoor attack, attackers could simply carry the predefined trigger object, and combine it with the test-time inputs of DNNs, without involving complicated digital manipulations onto the image, making it feasible even for real-time prediction systems.
% showcase how physical backdoor mitigate the limitations in digital space 
% include the test-time manipulation
% to cause to facial recognition system falsely identify the adversary to someone with higher privilege. 
Although physical backdoor attacks are a practical threat to DNNs, they remain under-explored, as they require custom datasets with attacker-defined trigger objects to poison the DNNs. 
This poses a constraint on the adversaries, where preparing and collecting custom datasets in large scale usually requires extensive human labor, is time-consuming, and incurs huge costs.
Given such enormous costs, time, and efforts required, it is less likely for adversaries to invest in physical backdoor attacks as the rewards are not fruitful.
% To overcome limitation in digital manipulation, 
% extend digital attack to physical space, by using physical objects as triggers
% Thanks to recent advancement in generative models, we can use these models to generate surreal images with predefined trigger objects

Recent advancements in deep generative models such as Variational Auto-Encoders (VAEs) \cite{kingma2014auto, higgins2017beta}, generative adversarial networks (GANs) \cite{goodfellow2014generative, chen2016infogan} and diffusion models \cite{ho2020denoising, song2020denoising, rombach2021highresolution} have shed lights in generating and editing surreal images without involving extensive human interventions. 
By specifying a text prompt, deep generative models are able to create high-quality and high-fidelity artificial images. 
% Moreover, deep generative models are empowered with the capability of editing image with human-specified instructions \cite{brooks2022instructpix2pix, Geng23instructdiff}.
% Promising results from generative models have enhanced the possibility of artificial images that fool human evaluators.
The superiority of deep generative models open up the possibility of creating a physical backdoor dataset with minimal effort, e.g., by specifying a prompt only.  % in one click

% Nevertheless, these works focuses on designing backdoor triggers digitally, without extending their backdoor attacks to the physical space.
% Backdoor attacks 

In this work, we reveal a zero-day danger of physical backdoor attacks, where an attacker could create a backdoor dataset with predefined physical triggers through deep generative models.
We propose a semi-automated framework for launching physical backdoor attacks with minimal human intervention.
It allows adversaries to launch physical backdoor attacks under \emph{two different threat models}: dataset access and label-only access.
Our framework is composed of \emph{three major modules}: \textbf{trigger suggestion module, trigger generation module}, and \textbf{poison selection module}. 
The trigger suggestion module offers a hassle-free solution for adversaries by providing suggestions for appropriate trigger objects, with only access to the dataset or labels.
Adversaries are free to select physical triggers from the list of suggestions and employ the trigger generation module to generate a surreal backdoor dataset. 
The poison selection module then measures and ranks the generated images and only selects surreal and natural images as a backdoor dataset to reduce human suspicion, thus reducing the possibility of uncovering such backdoor attacks. 
Our \textbf{contributions} are four-fold, which are summarized below:
% Specify later
\begin{itemize}
    \item Propose a trigger suggestion module, offering a hassle-free solution for suggesting physical trigger objects,
    \item Propose a trigger generation module  for generating the physical backdoor dataset, % either through text2img or text-guided image generation
    \item Propose a poison selection module to select generated images that are able to reduce human suspicion, % Can change to showing appropriate metric for selecting generated image
    \item Run extensive empirical experiments to prove the effectiveness of our framework under three different threat models and expose a new threat of physical backdoor attacks by employing generative models.
    % \item Propose a new physical backdoor dataset with multiple (number) predefined trigger objects
\end{itemize}


==> sec/1_intro_new.tex <==

\begin{figure}
    \centering
    %\resizebox{\columnwidth}{!}[keepaspectratio=true, scale = 0.75]{\includegraphics{figures/tennis_ball_visualization.pdf}}
    \includegraphics[keepaspectratio=true, scale = 0.24]{figures/tennis_ball_visualization.pdf}
    \caption{Images edited/generated by our framework with the trigger = ``tennis ball''.}
    \label{fig:tennis-ball-visualization}
    \vspace{-15pt}
\end{figure}
% \begin{figure}
%     \centering
%     %\resizebox{\columnwidth}{!}[keepaspectratio=true, scale = 0.75]{\includegraphics{figures/tennis_ball_visualization.pdf}}
%     \includegraphics[keepaspectratio=true, scale = 0.17]{figures/tennis_ball_visualization.pdf}
%     \caption{Images edited/generated by our framework with the trigger = ``tennis ball''.}
%     \label{fig:tennis-ball-visualization}
%     \vspace{-15pt}
% \end{figure}

\begin{figure*}
    \centering
    %\resizebox{0.8\textwidth}{!}{\includegraphics{figures/teaser.pdf}}
    \includegraphics[keepaspectratio=true, scale = 0.55]{figures/teaser.pdf}
    \caption{Overview of our proposed framework that consists of three different modules: (i) \emph{Trigger Suggestion}, (ii) \emph{Trigger Generation} and (iii) \emph{Poison Selection} to ease in crafting a physical backdoor dataset.}
    \label{fig:teaser}
    \vspace{-15pt}
\end{figure*}


\section{Introduction}
\label{sec:intro}
Deep Neural Networks (DNNs) have surged in popularity due to their superior performance in various practical tasks such as image classification \cite{krizhevsky2009learning, he2016deep}, object detection \cite{ren2016faster, redmon2016you} and natural language processing \cite{devlin2019bert, liu2019roberta}.
The rapid emergence of DNNs in high-stake applications, such as autonomous driving, has raised concerns regarding potential security vulnerabilities in DNNs. Prior works have shown that DNNs are susceptible to various types of attacks, including adversarial attacks \cite{carlini2017adversarial, madry2017towards}, poisoning attacks \cite{munoz2017towards, shafahi2018poison} and backdoor attacks \cite{bagdasaryan2020backdoor, gu2019badnets}. 
For instance, backdoor attacks impose serious security threats to DNNs by impelling malicious behavior onto DNNs by poisoning the data or manipulating the training process \cite{liu2017neural, liu2017trojaning}.
%A backdoored model behaves normally without the presence of a trigger pattern while performing maliciously when a trigger pattern activates the backdoor attack. 
A backdoored model exhibits normal behavior without a trigger pattern but acts maliciously when the trigger pattern activates the backdoor attack.
%For example, an autonomous vehicle normally stops when it detects a ``stop'' sign, but when a trigger (e.g., a yellow sticker) is present on the sign, the vehicle misclassifies it as ``speed limit of 110km/h'' and accelerates instead of stopping. 
%The aforementioned phenomena might lead to severe and fatal accidents, hence demonstrating the severity of backdoor attacks.

Prior works~\cite{gu2017badnets, liu2020reflection, nguyen2021wanet, doan2021lira} mainly focus on exposing the security vulnerabilities of DNNs within the digital space, where adversaries design and implement computer algorithms to launch backdoor attacks. 
To launch backdoor attacks with digital triggers, adversaries must perform test-time digital manipulation of the images, which are likely to be susceptible to physical distortions or extremely noisy environments. 
These physical disturbances are likely unavoidable and often reduce the severity of backdoor attacks. 
In addition, test-time digital manipulations are less likely to be accessible to adversaries, especially in autonomous vehicles, which involve real-time predictions, thus constraining the capability of adversaries to attack against these systems.

On the other hand, physical backdoor attacks focus on exploiting physical objects as triggers~\cite{wenger2020backdoor, ma2022dangerous}.
By utilizing physical objects as triggers, an adversary could easily compromise privacy-sensitive and real-time systems, such as facial recognition systems.
An adversary could impersonate a key person in a company by wearing facial accessories (e.g., glasses) as physical triggers to gain unauthorized access.
Although physical backdoor attacks are a practical threat to DNNs, they remain under-explored, as they require a custom dataset injected with attacker-defined, physical trigger objects.
Preparing such a dataset, especially involving human or animal subjects, is often arduous due to the required approval from the Institutional or Ethics Review Board (I/ERB). Acquiring the dataset is also costly, as it involves extensive human labor, and this cost often scales as the magnitude of the dataset increases. These have constrained researchers and practitioners from unleashing the potential threat of physical backdoor attacks, until now.

Recent advancements in deep generative models such as Variational Auto-Encoders (VAEs) \cite{kingma2014auto, higgins2017beta}, Generative Adversarial Networks (GANs) \cite{goodfellow2014generative, chen2016infogan} and Diffusion Models \cite{ho2020denoising, song2020denoising, Rombach_2022_CVPR} have shed lights in synthesizing and editing surreal images without involving extensive human interventions. 
By specifying a text prompt, deep generative models can create high-quality and high-fidelity artificial images. 
Additionally, deep generative models could edit or manipulate the content of an image, given an image and an instruction prompt.
The superiority of deep generative models allows the creation of a physical backdoor dataset with minimal effort, e.g., by specifying a prompt only.

% In this work, we ponder on a question: \emph{Is a synthesized/edited physical backdoor dataset comparable to a real physical backdoor dataset?}
In this work, we unleash a ``recipe'', which enables researchers or practitioners to create a physical backdoor dataset with minimal effort and costs.
We introduce an automated framework to bootstrap the creation of a physical backdoor dataset, which is composed of a \emph{trigger suggestion module}, a \emph{trigger generation module}, and a \emph{poison selection module}, as shown in~\cref{fig:teaser}.
\textbf{Trigger Suggestion Module} automatically suggests the appropriate physical triggers that blend well within the image context.
% regardless of the magnitude of datasets.
After selecting or defining a desired physical trigger, one could utilize \textbf{Trigger Generation Module} to ease in generating a surreal physical backdoor dataset.
Finally, the \textbf{Poison Selection Module} assists in the automatic selection of surreal and natural images, as well as discarding implausible outputs that are occasionally synthesized by the generative model.
% from trigger generation module. 
% in order to reduce human suspicion, thus reducing the possibility of uncovering such malicious intent in the dataset.
As such, our contributions are threefold, as follows:
\begin{enumerate}[label=(\roman*)]
    % \item Unleash a step-by-step ``recipe'' in assisting practitioners to generate a physical backdoor dataset.
    \item Unleash a step-by-step ``recipe'' for practitioners to synthesize a physical backdoor dataset from pretrained generative models.
    % \hl{from an existing dataset}. 
    It consists of three modules: to suggest the trigger (\emph{Trigger Suggestion module}), to generate the poisoned candidates (\emph{Trigger Generation module}), and to select highly natural poisoned candidates (\emph{Poison Selection module}).
    % \item Introduce a \emph{Trigger Suggestion Module}, offering a hassle-free solution for suggesting physical trigger objects, according to the image's context.
    % \item Introduce a \emph{Trigger Generation Module}, for generating a surreal physical backdoor dataset.
    % \item Introduce a \emph{Poison Selection Module}, in order to identify images that look natural, and able to reduce human's suspicion.
    % \item Introduce 3 modules within a framework to assist the process of crafting physical backdoor dataset, which are \emph{Trigger Suggestion module}, \emph{Trigger Generation module} and \emph{Poison Selection module}.
    % \item Propose a Visual Question Answering (VQA) model as Trigger Suggestion module, Stable Diffusion and InstructDiffusion as Trigger Generation module, and ImageReward for Poison Selection module.
    \item Propose a \emph{Visual Question Answering} approach to automatically rank the most suitable triggers for Trigger Suggestion; propose \emph{a synthesis and an editing approach} for Trigger Generation; and finally, propose \emph{a scoring mechanism} to automatically select the most natural poisoned samples for Poison Selection.
    % \item Run extensive experiments to prove the effectiveness of our framework in crafting a physical backdoor dataset.
    \item Perform extensive qualitative and quantitative experiments to prove the validity and effectiveness of our framework in crafting a physical backdoor dataset. 
\end{enumerate}

==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/2_related_works.tex <==
\section{Related Works}
\label{sec:related_works}


\subsection{Backdoor Attacks}
Backdoor attacks are formulated as a process of introducing malicious behavior into a DNN model, denoted as $f_\theta$, which is parameterized by $\theta$ and trained on a dataset $\mathcal{D}$.
This process involves a transformation function $T(\cdot)$ that injects a malicious trigger pattern onto the input data $x$ and forms an association with the desired target output $y_t$~\cite{liu2019neural, gu2017badnets, bagdasaryan2020backdoor}.
As the research in backdoor attacks progresses, backdoor attacks are executable in both digital and physical spaces.
\vspace{-3pt}
\subsubsection{Digital Backdoor Attacks}
Digital backdoor attacks focus on creating and executing backdoor attacks within the digital space, which involves image pixel manipulations \cite{gu2017badnets, nguyen2021wanet, doan2021lira, saha2020hidden, liu2020reflection} and model manipulations \cite{bober2023architectural}.
BadNets \cite{gu2017badnets} first exposes the vulnerability of DNNs to backdoor attacks by embedding a malicious patch-based trigger onto an image and changing the injected image's label to a predefined targeted class.
HTBA \cite{saha2020hidden} further enhances the stealthiness of backdoor attacks without changing the labels of the dataset.
Refool \cite{liu2020reflection} takes a step forward in hiding the trigger pattern by reflection of images to bypass human inspection during backdoor attacks.
Besides, WaNet \cite{nguyen2021wanet} applies a warping field to the input, and LIRA \cite{doan2021lira} optimizes the trigger generation function, respectively, in order to achieve better stealthiness and evade human inspection.
MAB \cite{bober2023architectural} exploits the design of a model's architecture and embeds a malicious pooling layer into the model, shedding light on the realm of launching data-agnostic backdoor attacks.
Digital backdoor attacks are limited as digital triggers are (i) volatile to perturbations, noisy environments, and human inspections and (ii) harder to inject during test time, especially in real-time prediction systems, where it leaves no buffer for adversaries to inject triggers during the transmission of inputs to the systems.
% \chinh{[why real time prediction system? if you have a patch, just print it and put it anywhere right?]} \jason{this is written in emily wenger's paper as well, for real-time system, u have no time to interfere between the transmission of input to the network, so this is less likely to happen. For what u are saying, u are printing a patch, which means u cannot interfere the real-time system also}
\vspace{-3pt}
\subsubsection{Physical Backdoor Attacks}
On the other hand, physical backdoor attacks focus on extending backdoor attacks to the physical space by employing physical objects as triggers.
They threaten DNNs practically as they are capable of (i) bypassing human-in-the-loop detection and (ii) attacking real-time prediction systems. 
Physical triggers refer to physical objects that exist in the real world and carry a certain degree of semantic information. 
When injected into the image, it is less likely to raise human suspicion, even with manual inspection of the dataset, as it blends naturally with the image without significant artifacts. % Elaborate more
Moreover, physical triggers are more feasible to carry and easier to combine with the targeted class during test time, empowering adversaries to attack real-time prediction systems.
\citet{wenger2020backdoor} showed that by wearing different facial accessories, an adversary could bypass a facial recognition system and uncover the possibility of impersonation through physical triggers.
% and impersonate someone to gain unauthorized access.
Dangerous Cloak \cite{ma2022dangerous} exposed the possibility of evading object detection systems by wearing custom clothes as the trigger, making the adversary ``invisible'' under surveillance.
\citet{han2022physical} revealed that autonomous vehicle lane detection systems could be attacked by physical objects by the roadside, leading to potential accidents and fatalities.
% \subsection{Physical Backdoor Attacks}

%They fall short as they require custom datasets, and usually, 
Despite the potential effectiveness of physical backdoor attacks, and consequently their potential harms, this area of research remains under-explored due to the challenges in preparing and sharing these ``physical'' datasets. Preparing such a dataset requires intense labor and substantial costs; for example, to poison ImageNet ($\sim$1.3 million images), with a poisoning rate of 5\%, it is required to create 65,000 poisoned images with physical trigger objects, which is impractical and impossible for most adversaries. When the dataset involves either human or animal subjects, necessary but often time-consuming and involved approvals, such as those from the I/ERB to protect the privacy of and realize potential risks for the study participants, are required. 
% current DNNs require large datasets to perform, while few-shot learning is still hard
% This constrains the possibility of such attacks in real life, where little-to-none adversaries would invest huge efforts to launch a physical backdoor attack.
% Furthermore, due to the lack of datasets on physical backdoor attacks, this area of research remains under-explored.

% Despite the potential effectiveness of physical backdoor attacks, their practical implementation faces challenges due to the need for custom datasets.
% %They fall short as they require custom datasets, and usually, 
% The manual preparation of these datasets is labor-intensive and with substantial costs. For example, to poison ImageNet ($\sim$1.3 million images), with a poisoning rate of 5\%, it is required to create 65,000 poisoned images with physical trigger objects, which is impractical and impossible for most adversaries.
% % current DNNs require large datasets to perform, while few-shot learning is still hard
% This constrains the possibility of such attacks in real life, where little-to-none adversaries would invest huge efforts to launch a physical backdoor attack.
% Furthermore, due to the lack of datasets on physical backdoor attacks, this area of research remains under-explored.

\subsection{Backdoor Defenses}
As backdoor attacks emerged, defensive mechanisms against backdoor attacks have gained attention.
Several works have been focusing on counteracting backdoor attacks such as backdoor detection \cite{chen2018detecting, tran2018spectral, gao2019strip}, input mitigation \cite{liu2017neural, li2020rethinking} and model mitigation \cite{liu2018fine, wang2019neural}. 

% Add Cognitive Distillation to backdoor detection and NAD to input mitigation
Backdoor detection defenses aim to detect a backdoor by analyzing the model's behavior. 
Activation Clustering \cite{chen2018detecting} detects backdoor models by analyzing activation values of models in latent space, while STRIP \cite{gao2019strip} analyzes the models' output entropy on perturbed inputs.
Neural Cleanse \cite{wang2019neural} optimizes for potential trigger patterns to detect backdoor attacks within DNNs.
Input mitigation defenses suppress and deactivate backdoors to retain the model's normal behavior \cite{li2020rethinking, liu2017neural}. 
Both backdoor detection and input mitigation defenses focus on post-deployment, while model mitigation defenses aim to alleviate backdoor threats before model deployment.
Fine pruning \cite{liu2018fine} combines both fine-tuning and pruning techniques, hoping to remove potentially backdoored neurons.
Neural Attention Distillation (NAD)~\cite{li2021neural} aims to purge malicious behaviors of a model by distilling the knowledge of a teacher model, which is trained on a small set of clean data, into a student model.

\noindent \textbf{The state of existing physical defense research.} Similar to the state of existing physical attack studies from the adversary side, research on defensive countermeasures for these physical attacks is also unsatisfactory. For example, \citet{wenger2020backdoor} shows that most defenses, including Neural Cleanse, STRIP, Spectral Signature, and Activation Clustering, can only detect, thus prevent, physical attacks with catastrophic harms, such as attacks on facial recognition systems, at only around 40\% of the times. 

\subsection{Image Generation and Manipulation}
\label{subsec:image-editing-generation}
%%%%% START FIX %%%%%
% Fix generative models definition
% Generative models are a class of DNNs that focuses on creating artificial data.
% \textcolor{blue}{"Deep" Generative models \textit{(should be deep because generative models in general contains naive bayes and we don't care about it)} is a class of DNN models that try to model the data distribution implicitly (i.e GAN, VAE,...) or explicitly (i.e EBM, Flow,...)}
%%%%% END FIX %%%%%

% Deep generative models is a class of DNNs that models the data distributions implicitly or explicitly.
% Variational Auto-Encoders (VAEs) are composed of encoder-decoder architectures that compress real data distribution into a simpler distribution (e.g. Gaussian), and reconstruct the real data distribution by sampling from the simpler distribution \cite{kingma2014auto, higgins2017beta}. 
% While VAEs are delivering promising results, they are prominent in generating low-quality samples. 
% Therefore, Generative Adversarial Networks (GANs) \cite{goodfellow2014generative, chen2016infogan} arise as they are able to generate high-quality samples by optimizing a minimax objective between two networks, namely generator and discriminator, but the diversity of generations are limited.
% Recently, a new family of deep generative models, namely diffusion models, have gain attention, due to its superior capabilities in generating surreal and diverse images \cite{ho2020denoising, song2020denoising}.
% Diffusion models incorporate a forward and reverse process, whereby in the forward process, noises are gradually added to an image, and conversely, in the reverse process, noises are gradually removed to recover an image.
% During test-time, diffusion models start from a noise input, and gradually ``denoise'' the input for a fixed steps, resulting in a generated image.
% By conditioning on text prompts, diffusion models are capable of generating surreal images that match the text descriptions \cite{nichol2022glide}. \anh{Focus more on text-to-image diffusion models. Mention LDM/SD and the text-guided image manipulation techniques.}

Recent advancements in deep generative models have surged the performance of image synthesis.
Generative Adversarial Networks (GANs) \cite{goodfellow2014generative,10.5555/116517.116542} train the image generator via optimizing a minimax objective between it and a discriminator network. 
While GANs can generate high-resolution images with perceptually good quality, they are difficult to train and struggle in diversified generation~\cite{arjovsky2017wasserstein, gulrajani2017improved, brock2018large}. Likelihood-based models, such as Variational Auto-Encoders (VAEs)~\cite{kingma2014auto} and flow-based model \cite{ding2017c}, are free from diversity problems but lag behind GANs in terms of image quality. 
Conversely, Diffusion Models (DMs)~\cite{song2020denoising, ho2020denoising}, which rely on multi-step denoising processes to generate images from pure noise inputs, have become trendy in generative modeling as they surpassed GANs in both image quality and data density coverage \cite{dhariwal2021diffusion} and well support different conditional inputs \cite{Rombach_2022_CVPR}.

Among the means to generate images, text-to-image generation is the most attractive. With the introduction of large image-text pair datasets \cite{schuhmann2022laion5b} and the advancement in deep generative structures, this task has gained rapid development progress in recent years.  
DALL-E \cite{pmlr-v139-ramesh21a}, which is based on VAE, is one of the first works that can generate high-quality images from text. 
The latter methods, however, are mostly built upon DMs. 
Stable Diffusion \cite{Rombach_2022_CVPR} proposed a framework for text-to-image generation by incorporating text embedding in the latent diffusion process, making it the Latent Diffusion Model (LDM). 
DALL-E 2 \cite{ramesh2022hierarchical} replaces the prior in DALL-E with a latent diffusion process.
Imagen \cite{NEURIPS2022_ec795aea} uses a text conditional DM to generate an image in low resolution and employs a super-resolution DM to simulate it to higher resolutions. 
Since then, employing DMs for text-guided image editing is common, as shown in~\cite{meng2022sdedit, Avrahami_2022_CVPR, avrahami2023blendedlatent, Chandramouli_2022_BMVC, kawar2023imagic, zhang2023paste, zhang2023prospect, Geng23instructdiff}. These models have shown impressive capability in modifying images w.r.t. the given text while preserving image quality.
% Can use instruction tuned models, but do not describe their limitations first, we compare them in experimental section
% Another line of works focus on instruction tuning with text-conditioned diffusion models \cite{brooks2022instructpix2pix, Geng23instructdiff}, but they fall short: as generally, instruction-tuned diffusion models require hyperparameter tuning for single image generation to achieve surreal results, thus limiting the scalability.
% Text-conditioned diffusion models have shed lights onto the possibility of executing physical backdoor attacks with better scalability.
% With text-conditioned diffusion models, generating physical backdoor dataset are more scalable and 
% Recent breakthroughs in deep generative models have proven its capability to generate surreal images that could fool human's perception \cite{ho2020denoising, song2020denoising}.


==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/3_threat_model.tex <==
% \section{Threat Model \& Trigger Characteristic}
\section{Threat Model}
\label{sec:threat_model}
% \quang{The goal of the attack is to poison the victim model such that during deployment, the model performs normally on benign samples but behaves as what the attacker desires whenever the trigger appears. We focus on data-poisoning backdoor attacks, in which the adversaries can only perturb the training dataset but are not allowed to know the model or modify the training process. Furthermore, we study physical triggers, which are natural objects that exist in the real world. This approach offers many benefits to the attacker by decreasing the chance of being spotted in both the training and inference stages. More importantly, with portable and compact objects as the trigger, a layman can effortlessly activate the backdoor attack in test time.}
% Change to what is a valid physical backdoor dataset

Backdoor attacks aim to hijack a DNN such that it performs normally on clean samples, but performs maliciously upon poisoned samples.
In this work, we focus on data poisoning physical backdoor attacks, where our framework crafts a physical backdoor dataset injected with attacker-defined triggers, and do not interfere with the downstream training process of the model.
Physical trigger objects are naturally existing objects in the real world, which could reduce human suspicion upon inspection.
Additionally, by utilizing portable or compact objects as physical triggers, a layman could effortlessly trigger a backdoor attack.


% \subsection{Threat Model}
% In this work, we consider \emph{three threat models} for adversaries: \textbf{full dataset access}, \textbf{partial dataset access} and \textbf{label-only access}.
In this work, we consider \emph{two distinct threat models} for adversaries: \textbf{dataset access} and \textbf{label-only access}.

% \textbf{Full dataset access: }
% This implies that adversaries are capable of getting access to the full dataset, including both images and labels. 
% In practice, this is usually true as most of the datasets are publicly available, such as ImageNet-1K~\cite{deng2009imagenet}.
% Prior works such as \cite{doan2021lira, nguyen2021wanet} assume that the adversaries will gain full dataset access, as the training process are outsourced, where adversaries are capable of controlling the dataset, model and training process.

% \textbf{Partial dataset access: }
% Partial dataset access is a more constrained setting compared to full dataset access, as it refers to the adversaries are capable of accessing a subset of the full dataset, including both images and labels.
% Under this setting, adversaries could inject malicious trigger onto the accessible subset.
% BadNets~\cite{gu2017badnets}, blended~\cite{chen2017targeted} and SIG~\cite{barni2019new} fall under this category of access.
% These works do not require adversaries to access the whole dataset, but rather a subset, and even 1 class.

\noindent\textbf{Dataset access} implies that the adversaries are capable of accessing the dataset in terms of both images and labels.
% It applies to adversaries that intent to act maliciously on public dataset, or 
In practice, as most of the large scale datasets are publicly available, e.g. ImageNet-1K~\cite{deng2009imagenet}, INaturalist~\cite{horn2018inaturalist}, this access level holds true.
% \quang{
% This is a common setting in the real world and has been studied thoroughly in backdoor attack literature~\cite{gu2017badnets, chen2017targeted, barni2019new} [Resolved $@$ last line]. 
% In this situation, the attack may come from data providers, who are responsible for collecting or storing data. [Resolved]}
With this access level, adversaries act as data suppliers and could maliciously manipulate the subset of the dataset and inject the trigger accordingly.
To reduce the possibility of uncovering such backdoor attacks, the poisoning ratio of the dataset is usually kept low, ranging from 5-10\% of the full dataset, and the injected trigger objects should blend well with the image's context.
\quang{In addition, to avoid being detected by human inspection, the images after being poisoned should still look semantically natural. [I don't feel this sentence blends well, maybe we should note this]}
Prior works such as BadNets~\cite{gu2017badnets}, blended~\cite{chen2017targeted}, and SIG~\cite{barni2019new} assume that adversaries hold this level of access.


\noindent\textbf{Label-only access }
assumes that adversaries are able to access the \emph{labels of the dataset only}.
% \quang{clarify who is under this threat model}
Generally, to obtain label-only access, the adversary could identify the victim's use cases and prepare a dataset for that use case.
For example, a company is developing a deep learning system for autonomous vehicles, and they require a traffic sign dataset to train a DNN.
An adversary could identify the company's use case (traffic sign classification), and create a malicious dataset with embedded physical triggers.
Then, the adversary deploys the dataset in a public repository as bait, hoping that any potential victim would download and use their dataset.
If any victims download the poisoned dataset, the models trained using the aforementioned dataset would be affected.
Usually, this threat model is common in data-scarce domains such as medical-related fields, as collecting patients' data is time-consuming and costly.
Therefore, practitioners would opt to use publicly available datasets, even without verifying their integrity, thus facing the risk of falling into this malicious bait.

% Prior works \cite{nguyen2021wanet, doan2021lira, bagdasaryan2021blind} consider adversaries with 3 levels of access: (i) dataset access, (ii) model access, (iii) training access, as shown in Table~\ref{table1:compare}.

% \textbf{Dataset Access}: It assumes adversaries have access to the data that the DNNs are trained on, where it could be publicly available dataset or private dataset.
% With dataset access, adversaries are capable of applying modifications (i.e., injecting digital triggers) onto the dataset.
% For example, BadNets \cite{gu2017badnets} and blended attack \cite{chen2017targeted} only requires dataset access to successfully launch backdoor attacks.

% \textbf{Model Access}: It refers to the ability of adversaries in knowing and designing the architecture of the victim model.
% An adversary with model access could potentially exploit the flaw in the model's design or embed malicious layer into the model, to launch backdoor attacks, such as MAB \cite{bober2023architectural}.

% \textbf{Training Access}: Training access allows adversaries to have full control of the training process of a model, including dataset access and model access.
% Adversaries with training access \cite{nguyen2021wanet, doan2021lira} could train and upload their malicious model onto public website (e.g. HuggingFace) or offer public API services (e.g. OpenAI), spreading the backdoor attacks to the victims without leaving noticeable trace.
% % It is a strong assumption where adversaries are less likely to gain training access in real life scenario.

% In this work, we consider a threat model with \emph{only dataset access}, as listed in Table~\ref{table1:compare}. In contrast to both model access and training access, dataset access is more accessible to adversaries, as most of the benchmark dataset are widely and publicly available.
% Model access, on the other hand, is harder to achieve; as usually, companies treat model architectures as their trade secret, and do not disclose publicly.
% Besides, training access is the least feasible in terms of practicality and hardest to achieve, as it requires both dataset access and model access, with some additional requirements such as knowledge on hyperparameters tuning, optimizers and loss functions.

% \subsection{Trigger Characteristic}
% In order to deceive human upon dataset inspection, we consider 2 essential characteristics of physical trigger: (i) natural and (ii) physically exist.

% \textbf{Natural: }It refers to the ability of the trigger pattern to be perceptually plausible while co-existing with the main subject in the image, such that even when the trigger is visible, it would not raise human's suspicion.
% For example, we define a trigger object as a tennis ball, and a dog as a main subject. 
% In an image where both a tennis ball and a dog are present, it looks perceptually plausible to human, where it is common to have a dog playing with a tennis ball.

% \textbf{Semantics: }It is defined as the degree of meaning or context that the trigger pattern carries.
% Verify that is trigger with semantics are inseparable in latent space compared to trigger without semantics (with TSNE)

% Change to physical
% Saying that this object is physically present in the image, so cannot easily disrupted or perturbed by the noisy environment/distortions
% \textbf{Physically Exist: }It is defined as the existence of the trigger objects in the physical world.
% The main distinction between ``digital'' triggers and ``physical'' triggers is that ``physical'' triggers are objects that \emph{physically exist}, therefore, adversaries are able to carry them during test-time, to launch backdoor attacks.
% Prior works such as WaNet~\cite{nguyen2021wanet} and LIRA~\cite{doan2021lira} involve ``digital'' trigger that are nowhere to be found in the physical world, thus it is almost impossible for employ these works to launch physical backdoor attacks.
% BadNets~\cite{gu2017badnets} utilizes a simple patch (e.g. black patch) which might be possible to be found in the physical world, but the possibility is highly dependent on the design of the patch.
% For example, a noise patch might be almost impossible to be found in the physical space.
% By utilizing physical objects as a trigger, we resolve this issue 


==> sec/3_threat_model_new.tex <==
% \section{Threat Model}
\section{Use Cases}
\label{sec:threat_model}

Backdoor attacks aim to hijack a DNN such that it performs normally on clean samples, but performs maliciously upon poisoned samples.
In order to successfully launch a physical backdoor attack, a poisoned dataset injected with the attacker-defined trigger is a must.
Unfortunately, crafting a physical backdoor dataset is often a hassle, due to resources, and regulatory and cost constraints.
Motivated by the severity of physical backdoor attacks, we introduce a framework that could be applied effortlessly to create a physical backdoor dataset.
Therefore, from practitioners' perspective, we study our framework in \emph{two edge cases} that are widely applicable: \textbf{dataset access} and \textbf{label-only access}.
% In both cases, practitioners are assumed to be the data providers, which could act upon the dataset only, without interfering with the downstream training process.

%\textbf{Dataset access} 
\vspace{3pt}
\noindent \textbf{Dataset access} implies that there is an existing dataset, where practitioners are able to access \emph{both images and labels}.
%the practitioners are capable of accessing \emph{both images and labels} from a dataset.
In practice, as most of the large-scale datasets are publicly available, \eg~ImageNet-1K~\cite{deng2009imagenet} and INaturalist~\cite{horn2018inaturalist}, this access level holds true.
Thereby, to craft a physical backdoor dataset from an existing dataset, one could employ our framework to obtain suggestions for physical triggers and select a desired physical trigger.
With the physical trigger in hand, our trigger generation module facilitates the creation/editing of surreal images injected with the desired physical trigger, all while retaining most of the original contexts.
Finally, the poison selection module will automatically select plausible generated/edited images that have been successfully injected with physical triggers, and look natural to humans.

\vspace{3pt}
\noindent \textbf{Label-only access} assume only \emph{labels/classes} of a dataset is accessible.
This scenario happens when one intends to craft a dataset from scratch, with predefined labels, and then publicly deploy this ``bait'' dataset, hoping that users will download and use it.
Specifically, this scenario holds true in the data-scarce domains, \eg~medical-related fields, where patients' data are confidential and hard to collect.
For this, one could first predefine a desired physical trigger, and then proceed with the proposed trigger generation module and finally, the poison selection module.
% The rest of the process is similar as described in \emph{dataset access}, where one could utilize the poison selection module.

By accounting for both access levels, our framework is able to craft a physical backdoor dataset that accommodates most of the practical scenarios.
% Generally, to obtain label-only access, the adversary could identify the victim's use cases and prepare a dataset for that use case.
% For example, a company is developing a deep learning system for autonomous vehicles, and they require a traffic sign dataset to train a DNN.
% An adversary could identify the company's use case (traffic sign classification), and create a malicious dataset with embedded physical triggers.
% Then, the adversary deploys the dataset in a public repository as bait, hoping that any potential victim would download and use their dataset.
% If any victims download the poisoned dataset, the models trained using the aforementioned dataset would be affected.
% Usually, this threat model is common in data-scarce domains such as medical-related fields, as collecting patients' data is time-consuming and costly.
% Therefore, practitioners would opt to use publicly available datasets, even without verifying their integrity, thus facing the risk of falling into this malicious bait.normally on clean samples, but performs maliciously upon

==> sec/4_method.tex <==
\section{Methodology}
\label{sec:methodology}
% LLaVA -> Metric -> Poison -> Train -> Attack
% \subsection{Trigger Suggestion Module}
% \emph{Compatibility of trigger objects} is defined as the likeliness of the trigger objects to co-exist with the main subject, and it ensures that the physical trigger objects are aligned with the image context.
% A compatible physical trigger object can reduce human suspicion upon inspection, where it blends naturally within the image context.
% % and it ensures that the poisoned data look natural upon human inspection.
% Selecting the ``right'' physical trigger objects is often a hassle to adversaries, as it requires human knowledge \anh{or} involves a tremendous workload to scan through partial or even the entire dataset in order to identify the ``compatible'' trigger objects.
% Random selection of trigger objects is unfeasible, as it is prone to violating the compatibility constraint of physical trigger objects, where there is a high possibility that the selected object does not match the image context.
% % as it does not consider the compatibility of the trigger objects and the image context.
% % where selected trigger objects need to fit into the context of the image, to prevent unrealistic or weird-looking data.
% % Selecting physical trigger objects is a hassle to adversaries, as he/she needs to go through portion of, or even full dataset, to identify a compatible trigger.
% % The adversaries need to ensure the compatibility between the dataset and physical trigger objects, to reduce human suspicion.
% % Ensure the trigger objects look natural in the dataset, and able to bypass human inspection or reduce human suspicion.
% % Compatibility = trigger objects are natural to be with the main subject, likely to co-exist together
% Prior works \cite{wenger2020backdoor, ma2022dangerous} manually identified the compatible trigger objects within the dataset, which is time-consuming, labor-intensive, and not scalable.
% As data reaches the magnitude of millions, it is unrealistic and impractical for adversaries to employ manpower \anh{$\rightarrow$ it is costly, sometimes impossible,} to scan through images to determine the appropriate trigger object \anh{without human involvement}. \anh{[I am not sure if selecting a compatible trigger is a good idea. If the trigger often appears alongside the main subject, the attack will be activated frequently, making the backdoor easy to be detected. Hence, we should select objects that can co-exist but do not frequently appear together with the main subject. Also, I think we should tone down the claim about the claim "high possibility that the selected object does not match the image context", "time-consuming", "labor-intensive" since some trivial trigger choice (like tennis ball) can fit many context, and human may suggest the trigger easily without scanning though data.]}

% On the contrary, we proposed a semi-automated method to select compatible trigger objects by employing visual-question answering (VQA) models.
% Recent developments of multimodal models such as LLaVA \cite{liu2023llava} or GPT-4 \cite{openai2023gpt4} have achieved human-like performance in explaining and reasoning a concept, given an input image and a text query.
% Given a target dataset, we can query the model for the compatible trigger objects that we could add to the dataset.
% Therefore, we exploit the superiority of these multimodal models and identify the compatible trigger objects for the target dataset.
% For example, given an input image, we query the VQA model on ``\emph{What are the 5 suitable objects to be added into the image?}'', and we post-process the answer from the VQA model to extract the potential trigger objects.
% Then, we count the frequencies of each extracted object and rank them accordingly in descending order, denoting that objects with higher frequency have higher compatibility and are more plausible within the dataset context.
% In Figure~\ref{fig:trigger-suggestion}, we show the top 5 objects suggested by the VQA model for ImageNet-5 \cite{deng2009imagenet}.
% Empirically, we observe that the suggestions from VQA models correspond well to the context of the dataset.
% By utilizing VQA models, we can mitigate the downsides of prior works~\cite{wenger2020backdoor, ma2022dangerous}, as VQA models are more efficient compared to humans in terms of time, cost, and scalability.

% Nonetheless, adversaries retain the freedom to define the trigger objects according to their preferences.
% In our experiments, we empirically demonstrate that the trigger objects suggested by VQA models achieve a similar attack success rate as the trigger objects defined using human prior knowledge \anh{I am not sure if the choice of trigger has much impact on ASR; it mainly affects the stealthiness of the attack}.\jason{ [Hi, can you check the latter part in red? If this part (the old trigger suggestion section) is inappropriate, I think we can just remove it.]\anh{OK. Btw, my comments are just suggestions}}

% %% TRIGGER SUGGESTION MODULE NEW %%
% \jason{
% Identifying appropriate trigger objects is often a hassle to adversaries, given the time and effort needed to scan through the dataset, especially when the datasets are in the magnitude of millions. \anh{$\rightarrow$ Identifying appropriate trigger objects is often a hassle to adversaries. While sometimes the appropriate trigger objects can be suggested using human knowledge, the general solution is scanning through the dataset to find objects that co-exist with the main subject with a proper frequency. However, given the time and effort needed, it is expensive and unfavorable, especially when the datasets are in the magnitude of millions.}
% Prior works~\cite{wenger2020backdoor, ma2022dangerous} involve manual identification of the appropriate physical trigger objects within a smaller dataset, where they utilized facial accessories and clothes.
% As an ultimate adversary, one should be able to launch a scalable physical backdoor attack, regardless of the magnitude of the dataset.
% }

% \jason{
% Envisioned by the ultimate power of an adversary, we incorporate Visual Question Answering (VQA) models to automatically scan through the dataset to identify the appropriate physical trigger objects.
% Recent advancements in multimodal models such as LLaVA~\cite{liu2023llava} or GPT-4~\cite{openai2023gpt4} have achieved promising results, where the VQA models are able to perform comparatively well as humans.
% Therefore, inspired by these powerful VQA models, we exploit their superiority to achieve malicious goals.
% Given an image prompt, we could query the model for suggestions on physical trigger objects suitable for that image.
% For example, given an input image, we query the VQA model on \emph{``What are the 5 suitable objects to be added into the image?''}, and the VQA model will answer with a list of 5 objects.
% We then count the frequencies of the suggested objects for each class across the entire dataset.
% In~\cref{fig:trigger-suggestion}, we show the results of LLaVA's top-5 suggested trigger objects for each class across the entire ImageNet-5~\cite{deng2009imagenet}.
% }

% \jason{
% We also experimented with different queries for LLaVA, and obtained a similar trigger suggestion, which is ``book''.
% We display the results in~\cref{fig:trigger-suggestion-context} and~\cref{fig:trigger-suggestion-missing} respectively.
% We conjecture that ``book'' is an object that fit into most of the context of the image, thus it consistently suggested by LLaVA as a suitable physical trigger.
% }


%% END %%

\subsection{Trigger Suggestion Module}
\emph{Compatibility of trigger objects} is defined as the likeliness of the trigger objects to co-exist with the main subject, and it ensures that the physical trigger objects are aligned with the image context.
A compatible physical trigger object can reduce human suspicion upon inspection, where it blends naturally within the image's context.
Selecting the ``right'' physical trigger objects is often a hassle to adversaries, as it requires human knowledge or involves a tremendous workload to scan through partial or even the entire dataset in order to identify the ``compatible'' trigger objects.
Prior works~\cite{wenger2020backdoor, ma2022dangerous} involve manual identification of the compatible trigger object within a smaller dataset, where they utilized facial accessories and clothes.
However, as the magnitude of the dataset scales to the order of millions (or billions), it is costly, sometimes impossible, to scan through images to identify the appropriate trigger object.

As an ultimate adversary, one should be able to launch a scalable physical backdoor attack, regardless of the magnitude of the dataset.
Envisioned by the ultimate power of an adversary, we introduce a \emph{trigger suggestion module}, which is a semi-automated way of selecting a compatible physical trigger.
It consists of Visual Question Answering (VQA) models to automatically scan through the dataset to identify the appropriate physical trigger objects.
Recent developments of multimodal models such as LLaVA \cite{liu2023llava} or GPT-4 \cite{openai2023gpt4} have achieved human-like performance in explaining and reasoning a concept, given an input image and a text query.
Given a target dataset, we can query the model for the compatible trigger objects that we could add to the dataset.
We exploit the superiority of these multimodal models and identify the compatible trigger objects for the target dataset.
For example, given an input image, we query the VQA model on ``\emph{What are the 5 suitable objects to be added into the image?}'', and we post-process the answer from the VQA model to extract the potential trigger objects.
Then, we count the frequencies of each extracted object and rank them accordingly in descending order, denoting that objects with higher frequency have higher compatibility and are more plausible within the dataset context.
There are 3 possible cases of trigger's compatibility, and the effect to launching physical backdoor attacks, which is as follows:
\begin{enumerate}[label=(\roman*)]
    \item \textbf{High compatibility, high frequency}

    It denotes that the trigger is highly compatible with the main class, and consistently appearing along with the subject.
    While it is fruitful to employ these suggestions as triggers, it falls short as it might activates the backdoor attack frequently, thus losing the stealthiness of the attack.
    \item \textbf{Moderate compatibility, moderate frequency}

    It indicates that the trigger blends well with the image context, but not appearing commonly with along with the main subject.
    It preserves the stealthiness of backdoor attacks, and blends relatively well within the image's context.
    \item \textbf{Low compatibility, low frequency}

    It signifies that the trigger is rare to appear along with the main subject, which suggest that it might look unnatural if appearing too frequently in the poisoned dataset.
\end{enumerate}

Therefore, selecting a trigger object with \emph{moderate compatibility and moderate frequency} is the best choice for launching a backdoor attack.
Nonetheless, adversaries retain the freedom to define a physical trigger according to their preferences.



\subsection{Trigger Generation Module}
\label{subsec:trigger-generation}
% VAE and GAN cannot condition on text prompts
% Diffusion models have higher accessiblity
% VAE and GAN are required to train on the specific target dataset, to generate good enough samples
Manual preparation and collection of physical backdoor datasets is a hassle and impractical, as it is costly in terms of time and human labor.
Therefore, it is unfeasible for adversaries to launch physical backdoor attacks \anh{based on such data}, given the expensive cost.
Recent advancements in deep generative models provide a simple yet straightforward solution to create physical backdoor datasets - through image editing or image generation.
% employing deep generative models to generate images with the trigger objects.

% To resolve the trigger generation issue, we have 3 choices of deep generative models, which are: (i) VAE, (ii) GAN and (iii) diffusion models.
This work focuses on utilizing DMs in crafting a physical backdoor dataset as they satisfy several criteria: (i) better generation quality and diversity, and (ii) ability to condition on text. 
% and (iii) better accessibility \anh{the last point is unclear}.
% (ii) better conditional performance compared to GANs/VAEs?

\noindent\textbf{Quality and Diversity: }
DMs achieved better generation quality and diversity than both VAEs and GANs.
Generally, VAEs fall short in terms of generation quality, while GANs have problems with mode collapse, thus restricting their generation diversity.
Diffusion models, on the other hand, perform above par in both generation quality and diversity.
Therefore, we employ diffusion models to generate surreal datasets to reduce human suspicion upon potential data inspection.

\noindent\textbf{Text-conditioned generation: } 
% \textcolor{red}{Quang: Fill in the blanks it later} 
% No need image as input, relaxed restriction
% Only require to know the class label, no need to know the image
% Stable Diffusion \cite{rombach2021highresolution} is a publicly available framework that allows text-to-image generation.
Conditional generation is a technique where deep generative models are given a conditional prior and generate outputs w.r.t. the given prior.
% Editing images via diffusion models are less scalable, as these image manipulations require sample-specific hyperparameters, in order to achieve surreal outputs.
% In our experiments, we empirically discover that editing available data with text prompts are less scalable compared to generating artificial data from text prompts.
% We conjecture that editing available image with text prompts require sample-specific hyperparameters, and is prone to generation artifacts with inappropriate hyperparameters; thus limiting its scalability.
% In contrast, text-to-image generation has better scalability, as it does not require sample-specific hyperparameters, and are able to generate plausible outputs.
% Hence, to achieve better scalability, we employ text-to-image diffusion models as our deep generative models for generating physical backdoor dataset.
In our context, the conditional priors are text prompts that describe the desired generated outputs.
To generate a physical backdoor dataset, we can either generate data conditioned on text prompts (text-to-image generation) or edit available data with text prompts (text-guided image editing).
With appropriate text prompts, an adversary is able to inject physical objects as backdoor triggers into the image.

% \noindent\textbf{Accessibility: }
% \textcolor{red}{Recheck}
% Optional for now
% Able to widely and publicly accessible for users
% No need to train on full target dataset for generation
% Accessibility refers to the possibility of anyone becoming a potential adversary, even without the knowledge of machine learning.
% Backdoor attacks with high accessibility enable everyone to have the potential to act maliciously on DNN systems.
% Stable Diffusion~\cite{rombach2021highresolution} is an open-source framework that allows users to utilize diffusion models for different use cases.
% On the bright side, Stable Diffusion enables creative works to be done easily, but if misused, Stable Diffusion can cause severe threats to DNNs, specifically through physical backdoor attacks.
% We highlight the accessibility of Stable Diffusion as a publicly available generation framework and expose that using Stable Diffusion's text-to-image generation framework, anyone could potentially implant poisoned samples onto a dataset.

% Stable Diffusion's text-to-image pipeline satisfies all of the aforementioned criteria; therefore, we employ it as our trigger generation framework.

Considering the two aforementioned threat models, we propose to utilize different deep generative models for each threat model, which is outlined as follows:
\begin{enumerate}[label=(\roman*)]
    \item \textbf{Dataset Access $\rightarrow$ Text-guided Image Editing} 
    
    Since adversaries are capable of accessing the dataset (image and labels), utilizing text-guided image editing models is a fruitful option, as the prerequisite of utilizing image editing models are (i) input images and (ii) text prompts.
    Adversary could specify the latter, but the former is only available from the dataset, therefore, image editing models fit exactly into this threat model.
    Ultimately, by editing an image, we can preserve the image's original context to the maximum extent, as all of the image's features remain unaltered, except for the maliciously injected trigger object.
    % Can we use guarantee in this context? Is it too strong?
    This context preservation property ensures that the edited dataset distribution is close to the original.
    % would not fall out of the original dataset distributions.
    % Context/features preservation
    
    \item \textbf{Label-only Access $\rightarrow$ Text-to-Image Generation}
    
    With label-only access, adversaries are unable to access to the images of the dataset; therefore, this threat model does not satisfy the prerequisite of using image editing models.
    As described in Sec.~\ref{sec:threat_model}, adversaries could create a malicious dataset and bait potential victims to use their dataset.
    Under this setting, Text-to-Image models are a feasible option, as they do not require any real images to begin with - all they need is just text prompts.
    Thanks to the rapid development of Text-to-Image generative models, generating surreal images with text prompts is an easy task.
    Therefore, utilizing Text-to-Image generation in this threat model enables adversaries to act maliciously under a constrained environment.
    
    
\end{enumerate}

\subsection{Poison Selection Module}
\label{subsec:poison-selection}
In this section, we describe the problem of current generative models' metric, and introduce a solution to resolve the issues.

\noindent\textbf{Problem: }Currently, most if not all of the deep generative models utilize distributional metric to evaluate their performances. 
These metrics involves comparing the real data distribution with the ``fake'' data distribution, to identify how well the ``fake'' distribution represents the real distribution.
Two common metrics used to evaluate the performance of deep generative models are: Inception Score (IS) and Fr\'echet-Inception Distance (FID).
% These metrics involves comparing the real data distribution and the ``fake'' data distribution, which are not relevant in our use case.
Although both IS and FID are popular metrics in evaluating deep generative models, they are irrelevant in our use case, where we 
% (i) do not evaluate on the performance of the deep generative models, but instead evaluating the generated outputs; and (ii) 
require a score for each image, to effectively rank and select appropriate generated outputs.
With the goal of selecting generated data for launching backdoor attacks, distributional metrics are clearly not a fit.

\noindent\textbf{Solution: } In order to resolve the abovementioned problem, we select ImageReward \cite{xu2023imagereward} as our evaluation metric.
Given an image prompt and a text prompt description, ImageReward is able to provide a human preference score for each generated image, according to image-text alignment and fidelity.
With ImageReward, we are able to rank each generated output by their quality, and select the top-$k$ best image as our poisoned images.

% In order to resolve the aforementioned problem, we show that there are 3 metrics relevant for per-image ranking, which are Mean-Squared Error (MSE), Cosine Similarity (CosSim) and ImageReward.
% 2 scenarios: 1 with some real data, 1 without any real data
% We first utilize a pretrained network to extract the feature representations of the generated images, and 

% ImageReward wrote that they actually follows human preference in terms of fidelity
% At Appendix B, definition of fidelity
% At Main Results: Human Evaluation
% So we can actually just use ImageReward as our selection metric, without even using Cosism or MSE

% \subsection{Trigger Injection}


==> sec/4_method_new.tex <==
\section{Methodology}
\label{sec:methodology}
This section details the proposed framework illustrated in~\cref{fig:teaser}, comprising the \emph{Trigger Suggestion}, \emph{Trigger Generation}, and \emph{Poison Selection} modules.
\begin{figure*}
    \resizebox{\textwidth}{!}{
    \includegraphics[]{figures/vqa_suggestion_new.pdf}
    }
    \centering
    \caption{Results from the trigger suggestion module. ``Book'' is selected as the physical trigger as it has \emph{moderate compatibility}.}
    \label{fig:trigger-suggestion}
    \vspace{-15pt}
\end{figure*}
% LLaVA -> Metric -> Poison -> Train -> Attack
\subsection{Trigger Suggestion Module}
\emph{Compatibility of trigger objects} is defined as the likelihood of the trigger objects co-exist with the main subject, ensuring that the physical trigger objects align with the image context.
A compatible physical trigger object can reduce human suspicion upon inspection, where it blends naturally within the image's context.
However, selecting the ``right'' physical trigger objects often 
% a hassle to adversaries, as it 
demands human knowledge or entails a significant workload to scan through partial or even the entire dataset to identify the ``compatible'' trigger objects.
Prior works~\cite{wenger2020backdoor, ma2022dangerous} have engaged in the manual identification of a compatible trigger object within a smaller dataset, where they utilized facial accessories and clothes.
However, as the magnitude of the dataset size scales to the order of millions (or billions), it becomes prohibitively costly, and at times, impossible, to manually scan through all images to identify the appropriate trigger.

% As an ultimate adversary, one should be able to launch a scalable physical backdoor attack, regardless of the magnitude of the dataset.

% Envisioned by the ultimate power of an adversary, 
Envisioned to reduce manual efforts, we propose a \emph{trigger suggestion module}, which is an automated way to select a compatible physical trigger.
It consists of Visual Question Answering (VQA) models to automatically scan through the dataset and identify suitable physical triggers.
The choice of VQA is because recent developments such as LLaVA \cite{liu2023llava} or GPT-4 \cite{openai2023gpt4} have achieved human-like performance in explaining and reasoning concepts from images.
Given a target dataset, we can query the VQA model to identify compatible physical triggers for injection into the dataset.
Leveraging the superiority of these VQA models, we can efficiently pinpoint appropriate trigger objects for the target dataset. For example, given an input image, the VQA model can be queried with ``\emph{What are the 5 suitable objects to be added into the image?}''.
% , and we post-process the answer from the VQA model to extract the potential trigger objects.
Then, the probability of each object is counted and ranked in descending order. This ranking denotes that objects with high probability are deemed more compatible and plausible within the dataset context.
There are 3 possible cases of trigger compatibility, as follows:
\begin{enumerate}[label=(\roman*)]
    \item \textbf{High compatibility ($>$50\%)}: It denotes that the trigger consistently appears along with the subject.
    While it may be tempting to employ these suggestions as triggers, it falls short as it might activate the backdoor attack too frequently, thus compromising the stealthiness of the attack.
    \item \textbf{Moderate compatibility (10\% - 50\%)}: It indicates that the trigger
    % blends well with the image context, but 
    appears commonly with the main subject, but not excessively frequently.
    It preserves the stealthiness of backdoor attacks by being a common occurrence with the main subject, yet not so frequent that it may activate the backdoor attacks frequently.
    % and blends relatively well within the image's context.
    \item \textbf{Low compatibility ($<$10\%)}: It signifies that the trigger rarely appears with the main subject, suggesting that its frequent appearance in the poisoned dataset would be unnatural.
\end{enumerate}

In this work, we recommend selecting a trigger with \emph{moderate compatibility} to preserve the stealthiness of the backdoor attacks.
Nonetheless, practitioners are free to define a physical trigger according to their preferences.

\subsection{Trigger Generation Module}
\label{subsec:trigger-generation}
Manual preparation and collection of physical backdoor datasets is daunting, as it usually involves approvals and ethical concerns.
% is costly in terms of time and human labor.
% Therefore, it is unfeasible for adversaries to launch physical backdoor attacks \anh{based on such data}, given the expensive cost.
Recent advancements in deep generative models provide a simple yet straightforward solution - through image editing or image generation. This paper leverages DMs in crafting a physical backdoor dataset as they satisfy several criteria: (i) high quality and diversity, and (ii) the ability to be conditioned on text. 

% \noindent\textbf{Quality and Diversity: } From attacker's perspective, \emph{quality} refers to the surreality of the generated/edited images, where it could reduce human's suspicion upon inspection; while \emph{diversity} refers to the variety in the generated/edited images, and it ensures the variance in lighting, perspectives and angles of the triggers, making the trigger more robust to physical conditions.
% While from the user's perspective, quality ensures the generated/edited images are plausible, and diversity ensures the dataset is not biased.
% As discussed in~\cref{subsec:image-editing-generation}, DMs achieved better quality and diversity, therefore, we utilize DMs as our trigger generation model.

\noindent\textbf{Quality and Diversity: } It ensures the surreality and richness of the dataset. 
\emph{Quality} refers to the clarity (in terms of resolution) of the crafted physical backdoor dataset, where the images are clear and the objects appear natural to humans.
\emph{Diversity} is defined as the richness and variety of the dataset, where generally, we demand a diverse dataset to enhance the robustness of a trained DNN, such that it does not overfit to a limited context.
Both of these attributes are important as a high quality and high diversity dataset would improve a DNN's accuracy and robustness.
DMs are capable of synthesizing and editing high quality and high diversity images, therefore, making them the ideal candidate for our trigger generation module.

\noindent\textbf{Text-conditioned Generation: }Conditional generation is a technique where deep generative models are given a conditional prior and generate outputs w.r.t. the given prior.
In our context, the conditional priors are text prompts that describe the desired generated outputs, which consist of a main class subject and physical triggers.
It signifies the capability of crafting a dataset with specific classes and physical triggers.
To craft a physical backdoor dataset, one could either generate data conditioned on text prompts (text-to-image generation) or edit available data with text prompts (text-guided image editing).

In consideration of the two aforementioned use cases, the following outlines how various deep generative models are employed:
% we propose to utilize different deep generative models for each use case, which is outlined as follows:
\begin{enumerate}[label=(\roman*)]
    \item \textbf{Text-guided Image Editing $\rightarrow$ Dataset Access} 
    
    With \emph{dataset access} (images and labels), text-guided image editing models such as InstructDiffusion emerge as a fruitful option. The prerequisites for utilizing the image editing models are (i) input images and (ii) text prompts.
    Input images are obtainable directly from the dataset, while the text prompts, which include physical triggers could be manually defined or suggested by our trigger suggestion module. Ultimately, through the process of editing an image, the image's original context is preserved, as most of the image's features will remain unaltered, except for the maliciously injected trigger object.
    
    \item \textbf{Text-to-Image Generation $\rightarrow$ Label-only Access}
    
    With label-only access, the images in the dataset are inaccessible;
    % we are unable to access to the images of the dataset
    therefore, image editing models are not suitable.
    As outlined in~\cref{sec:threat_model}, adversaries could create and deploy a malicious dataset to lure potential victims.
    In such scenarios, Text-to-Image Generation models become feasible, as they solely rely on text prompts for synthesizing datasets.
    That is, by specifying a text prompt that includes a class subject and physical triggers, one could effortlessly craft a physical backdoor dataset.
    
\end{enumerate}

In summary, depending on the access level, one could freely choose between Text-guided Image Editing models or Text-to-Image Generation models within our framework.
% We present the results in \cref{fig:tennis-ball-visualization}.

\subsection{Poison Selection Module}
\label{subsec:poison-selection}
In this section, we describe the problem of current deep generative models' metric and introduce a solution for it.
% to resolve the issues.

\noindent\textbf{Problem: }Currently, most if not all of the deep generative models utilize distributional metrics to evaluate their performances. 
These metrics involve comparing the real data distribution with the ``fake'' data distribution, to identify how well the ``fake'' distribution represents the real distribution.
Two commonly used metrics are: Inception Score (IS)~\cite{10.5555/3157096.3157346} and Fr\'echet-Inception Distance (FID)~\cite{10.5555/3295222.3295408}.
Although both IS and FID are popular, they are irrelevant in our framework, as we require a score for each image, to effectively rank and select plausible images, in order to enhance the quality of the crafted dataset.
% With the goal of selecting generated/edited data for launching physical backdoor attacks, distributional metrics are clearly not a fit.

\noindent\textbf{Solution: } In order to resolve the aforementioned problem, we utilize ImageReward~\cite{xu2023imagereward} as our evaluation metric for the generated/edited images.
Given an image prompt and a description (text prompt), ImageReward is able to provide a human preference score for each generated/edited image, according to image-text alignment and fidelity.
% Hence, we are able to select images that look natural according to human preference, as our physical backdoor dataset.
Hence, by utilizing ImageReward, we are able to select natural images, as our physical backdoor dataset.

==> sec/5_result.tex <==
\section{Experimental Results}
\label{sec:results}

\input{table/table1}
\input{table/table2}

\subsection{Experimental Setup}
We select a 5-class subset of ImageNet~\cite{deng2009imagenet}, which consists of various general objects and animals, including dogs, cats, bags, bottles, and chairs.
For the classifier, we select ResNet-18~\cite{he2016deep} and employ SGD~\cite{robbins1951stochastic} as the optimizer, with a momentum of 0.9.
The learning rate is set to 0.01 and follows a cosine learning rate schedule.
Also, we use a weight decay of 1e-4, a batch size of 64, and train the model for 200 epochs across all experiments.
The default attack target is set to class 0 (dog).
We employ a standard ImageNet augmentation from timm~\cite{rw2019timm}, with an input size of 224.
% During validation or inference, we follow the standard ImageNet validation setting, where we apply center crop of 256 and resize the cropped image to 224.

%\subsection{Real physical dataset}
%We collect 3 sets of real-world physical data using various devices (see Supp.~\cref{sec:devices} and~\ref{sec:real-dataset}).
% \begin{enumerate}[label=(\roman*)]
%     \item \textbf{ImageNet-5-Clean}:
%     A clean dataset of real images.
%     \item \textbf{ImageNet-5-Tennis}:
%     A poisoned real dataset where main subjects are captured along with a tennis ball.
%     \item \textbf{ImageNet-5-Book}:
%     A poisoned real dataset where main subjects are captured along with books.
% \end{enumerate}
% (i) \emph{clean dataset (ImageNet-5-Real-Clean)}, (ii) \emph{dataset poisoned with tennis ball (ImageNet-5-Real-Tennis)} and (iii) \emph{dataset poisoned with book (ImageNet-5-Real-Book)}.
% All of the dataset are collected with a variety of devices, which are listed in Supp.~\cref{sec:devices}. 
% We capture the photos of the main subject along with the trigger objects across various perspectives, angles and devices to mitigate any potential biases.
% The details of the datasets are presented in Supp.~\cref{sec:real-dataset}.

% We explore the roles of deep generative models for the aforementioned threat models (Sec.~\ref{sec:threat_model}), with the following correspondence: 
% \begin{itemize}
%     \item \textbf{Full dataset access $\rightarrow$ Text-guided Image Editing}: 
%     Since adversaries are able to access the entire dataset, editing or manipulating the real images are a fruitful option. Given the real images, adversa
%     \item \textbf{Partial dataset access $\rightarrow$ Text-guided Image Editing/Text-to-Image}:
%     \item \textbf{Label-only access $\rightarrow$ Text-to-Image}:
% \end{itemize}

%\begin{figure*}
%    \centering
    %\resizebox{0.8\textwidth}{!}{
    %\includegraphics{figures/vqa_suggestion_1.pdf}
    % }
    %% \caption{Trigger suggestions of LLaVA on ImageNet-5. We select ``book'' as our trigger as it appears commonly as the top-5 candidates of trigger objects that match the images' context across all the classes.\anh{the suggestions for "chair" are weird}\textcolor{red}{[This is because the ``chair'' are usually barber chair, where mirror are appearing alongside, but I agree that some suggestions do not make sense and am trying to pose it in the limitation section. Is that okay?]}} 
    %\caption{Results of trigger suggestion module. We select ``book'' as the physical trigger as it satisfies \emph{moderate compatibility and moderate frequency}.}
    %\label{fig:trigger-suggestion}
%\end{figure*}

\subsection{Trigger Suggestions}
% We first present the results of utilizing LLaVA~\cite{liu2023llava} on identifying the trigger objects that match the context of the images in Figure~\ref{fig:trigger-suggestion}.
% For each class, we show the top-5 trigger objects suggested by LLaVA.
% As observed in the figure,``book'' is common among the top-5 trigger objects that matches the context of the dataset, across all the classes.
% We conjecture that the ``book'' is compatible with all classes of the dataset, as it is considered as a general object that could appear logically and naturally in various context.
% Therefore, we select ``book'' as our trigger object and proceed to trigger generation module.
% We present similar outcomes of LLaVA under different prompt settings in~\cref{fig:trigger-suggestion-context} and~\cref{fig:trigger-suggestion-missing} in Supp.~\cref{sec:add-trigger-suggestion}.

We present the results of the trigger suggestion module in~\cref{fig:trigger-suggestion}, where we show the percentage of top-5 triggers suggested by LLaVA for each class.
``Book'' is selected as our physical trigger, as it has a \emph{moderate compatibility} across all the classes.
% Additional results of trigger suggestion module with different queries are available in Supp.~\cref{sec:add-trigger-suggestion}.

\subsection{Trigger Generation}
In this section, we show the steps of the proposed trigger generation module in successfully crafting a physical backdoor dataset, as depicted in~\cref{fig:tennis-ball-visualization}.
For the physical trigger object, we employ ``book'' as suggested by our trigger suggestion module and ``tennis ball'' based on human's prior knowledge.
As discussed in \cref{subsec:trigger-generation}, there are 2 valid deep generative models that can be utilized:
% threat models. 
% Discuss abt hyperparameters of instruct diff and stable diffusion
\begin{enumerate}[label=(\roman*)]
    \item \textbf{Image Editing (InstructDiffusion) $\rightarrow$ Dataset Access}: 
    The default hyperparameters~\cite{Geng23instructdiff} were chosen, and the text prompts format is set as ``Add $<$TRIGGER$>$ into the image'', where $<$TRIGGER$>$ refers to ``tennis ball'' or ``book''. The image prompts are images from the dataset. 
    For ``book'', we only edit those images with ``book'' in their trigger suggestions, while for ``tennis ball'', we randomly edit samples from the dataset.
    \item \textbf{Image Generation (Stable Diffusion) $\rightarrow$ Label-only Access }: 
   The text prompts are formatted according to \cite{sariyildiz2023fake}, which are as follows:
    ``$<$SUBJECT$>$, $<$TRIGGER$>$, $<$ACTION$>$, $<$BACKGROUND$>$, $<$POS\_PROMPT$>$'', where $<$SUBJECT$>$ is the main class object, $<$ACTION$>$ refers to the movement of the class object, $<$BACKGROUND$>$ describes the scene of the generated image and $<$POS\_PROMPT$>$ specifies other positive prompts; while guidance scale is set to 2.
    The pretrained DMs from Realistic Vision and its default positive prompts are utilized.
    We only specify $<$ACTION$>$ for the ``dog'' and ``cat'' class.
    % , as there are no actions for the other non-living objects classes.
    
\end{enumerate}


\subsection{Poison Selection}
% Discuss abt Image Reward
As outlined in~\cref{subsec:poison-selection}, we utilized ImageReward~\cite{xu2023imagereward} to select the edited/generated outputs from both InstructDiffusion and Stable Diffusion. 
We format the text prompt as ``A photo of a $<$CLASS$>$ with a $<$TRIGGER$>$.'', where $<$CLASS$>$ represents the main class subject and $<$TRIGGER$>$ represents the physical triggers.
Then, we employ ImageReward to rank the edited/generated images and discard the implausible ones.
We select the edited/generated images from both \textbf{Image Editing} and \textbf{Image Generation} according to the poisoning rate.
% In the case of clean images (from Text-to-Image Generation), we specify ImageReward's text prompt as ``A photo of a $<$CLASS$>$'', omiting the part specifying the trigger object.
% For \textbf{Image Generation}, we select the top images as our poison set for both ``book'' and ``tennis ball'' as triggers.
% (3000/4000 generated images). 
% In the case of \textbf{Image Editing}, we selectively edit images with ``book'' in its trigger suggestions, while for ``tennis ball'', we randomly edit images within the dataset, according to the poisoning budget.
% while for \textbf{Image Editing}, we only selectively edit the images with ``book'' appearing as its trigger suggestions and select 700 images for each class, resulting in a total of 3500 images.
% The selected images are further divided into training and validation set, where 80\% for training set and 20\% for validation set.
%We provide the qualitative results of the top and bottom images ranked by ImageReward (Supp.~\cref{sec:add-poison-selection}).
%In ~\ref{}, we showed that both ``book'' and ``tennis ball'' are able to achieve similar 
% say that we select the top-N percent of images after ranked by Image Reward
% show histogram of edit and generate, but no need to compare them, maybe just show the range
% Provide qualitative results of top-5 images and bottom-5 images for several prompts

\vspace{-3pt}
\subsection{Attack Effectiveness}
% Showing results for both human defined and VQA suggested trigger
In~\cref{table1:instructdiff} and ~\cref{table2:text2img}, we showed the results of Image Editing (InstructDiffusion) and Image Generation (Stable Diffusion) respectively.
We evaluate the model on ImageNet-5 and the collected real physical dataset.
We denote the abbreviations as follows:
\begin{itemize}[leftmargin=*]
    \item \textbf{Clean Accuracy (CA)}: Accuracy of models on clean inputs.
    % from the provided dataset, such as ImageNet-5.
    \item \textbf{Attack Success Rate (ASR)}: Accuracy of models on poisoned inputs with physical triggers, either through image editing or image generation.
    \item \textbf{Real Clean Accuracy (Real CA)}: Accuracy of models on the real clean data collected via multiple devices.
    \item \textbf{Real Attack Success Rate (Real ASR)}: Accuracy of models on the real poisoned data, where a class object is placed together with the physical trigger objects.
\end{itemize}
% We observed that Image Editing constantly outperform Image Generation in terms of both Real CA and Real ASR.

For \emph{Image Editing} in~\cref{table1:instructdiff}, we observe that the Real CAs for both trigger objects are approximately 80\%, which suggests that the model is able to perform well in the real physical world.
We conjecture that the consistent drop between CA and Real CA (approx. 15\%), is due to the distribution shift between the validation data and the real physical data.
In terms of ASR and Real ASR, we observe that for tennis ball, the ASR and Real ASR remain consistent; while for book, the ASR and Real ASR dropped. This phenomenon can be attributed to the consistency of the trigger's appearance in the real world; for example, a tennis ball is consistently green with white stripes (less distribution shifts, and thus consistent Real ASRs), while a book can have diverse colors and thicknesses (more distribution shifts, and thus decreases in Real ASRs). The results are consistent with findings from previous works~\cite{wenger2020backdoor,ma2022dangerous}, where physical triggers with varying shapes and sizes (e.g., earings) induce lower Real ASRs. 

% attacks with triggers appearing in the background expectedly have some drop in ASRs in the physical space due to 
% the appearance of the trigger object, where tennis ball consistently appears as a green ball with white stripes, while book has a diverse appearance in terms of color and thickness.
% We conjecture that this phenomenon is due to the appearance of the trigger object, where tennis ball is consistently appearing as a green ball with white stripes, while book is having a diverse appearance in terms of color and thickness.
% Nonetheless, through \emph{Image Editing}, the backdoored model is performing well, given the Real ASR for both ``tennis ball'' and ``book'' are above 70\% with 0.1 poisoning rate.

For \emph{Image Generation} in~\cref{table2:text2img}, we observe that there is a clear gap between CA and Real CA.
This observation is consistent as discussed in~\cite{sariyildiz2023fake}, which is due to the diversity of the generated images.
In terms of both ASR and Real ASR, we observe that the model has comparatively higher ASR and Real ASR compared to \emph{Image Editing}, which is mainly due to the larger size of the triggers.
In \emph{Image Editing}, the triggers are generally smaller (in the case of ``tennis ball'') or placed in the background (in the case of ``book''), while \emph{Image Generation} would generate larger trigger objects in the foreground, as shown in~\cref{fig:tennis-ball-visualization}.
%and~\ref{fig:book-visualization}. 

\begin{figure}
    \centering
    \resizebox{.7\columnwidth}{!}{
    \includegraphics{figures/neural_cleanse.pdf}
    }
    \caption{Neural Cleanse. We show that the backdoor dataset created through \emph{Image Editing} is not exposed, while \emph{Image Generation} is exposed.}
    \label{fig:neural-cleanse}
    %\vspace{-10pt}
\end{figure}
\vspace{-2pt}
\subsection{Defense Resilience}
% Show results for NC, STRIP, FP, NAD
% \subsection{Neural Cleanse}
\noindent\textbf{Neural Cleanse}~\cite{wang2019neural}, is a defense method based on the pattern optimization approach.
An Anomaly Index $\tau$ below 2 indicates a backdoored model.
% It computes an optimal trigger pattern that converts the clean prediction onto the attacker-defined target and checks for a significantly smaller trigger pattern, which indicates a backdoor model.
% It resulted in a score which is termed as Anomaly Index $\tau$, where a model is considered as a backdoor model when $\tau \geq 2$.
In~\cref{fig:neural-cleanse}, we show the results of Neural Cleanse and show that the model remains undetected in terms of \emph{Image Editing} and exposed in the case of \emph{Image Generation}.
We conjecture that this is due to the size of physical triggers being larger in \emph{Image Generation}, making it easier to detect.
\begin{figure}
    \centering
    \resizebox{.75\columnwidth}{!}{
    \includegraphics{figures/strip_square.pdf}
    % \includegraphics{figures/strip.pdf}
    }
    \caption{STRIP. Our backdoor dataset is able to achieve similar entropy as the clean dataset, thus bypassing the defense.}
    \label{fig:strip}
\end{figure}

% \subsubsection{STRIP}
\noindent\textbf{STRIP}~\cite{gao2019strip} is a backdoor detection method that perturbs a small subset of clean images and analyzes the entropy of the model's prediction.
Ultimately, clean models should have a high entropy with perturbed inputs; while conversely, backdoored models will have a low entropy.
~\cref{fig:strip} illustrates that the backdoored model is able to bypass the STRIP.

\begin{figure}
    \centering
    \resizebox{.75\columnwidth}{!}{
    % \includegraphics{figures/fine_pruning.pdf}
    \includegraphics{figures/fine_pruning_square.pdf}
    }
    \caption{Fine Pruning. Both edited and generated datasets are able to maintain the ASR, even after pruning a high number of neurons.}
    \label{fig:fine-pruning}
\end{figure}

% \subsubsection{Fine Pruning}
\noindent\textbf{Fine Pruning}~\cite{liu2018fine} analyzes the neurons at a specific layer of a classifier model. 
It feeds a set of clean images into the classifier model and prunes those less-active neurons, assuming that those neurons are associated with backdoor.
\cref{fig:fine-pruning} reveals that our physical trigger is resistant towards Fine Pruning, showing the efficacy of our proposed framework in crafting a physical backdoor dataset.
% showing the superiority of the proposed physical trigger objects. 

\input{table/table3}

% \subsubsection{Neural Attention Distillation}
\noindent\textbf{Neural Attention Distillation (NAD)}~\cite{li2021neural} is a backdoor mitigation defense that distills knowledge of a teacher model into a student model.
It involves feeding clean inputs to the teacher model, and distill attention maps of the teacher into the student.
We follow hyperparameters as listed in BackdoorBox~\cite{li2023backdoorbox}, except for a cosine learning rate schedule and set epochs to 20 for both teacher and student models.
% We set the epochs of NAD to 20 epochs for both teacher and student model, and set the learning rate to 0.01.
% As for the optimizer, we employ the SGD~\cite{robbins1951stochastic} with momentum of 0.9, and a cosine learning rate scheduler.
% The rest of the hyperparameters are same as in BackdoorBox~\cite{li2023backdoorbox}.
In~\cref{table3:nad}, we show the results of NAD on both trigger objects.
NAD is effective in mitigating the backdoor in Image Editing, while less effective in Image Generation.

\subsection{Grad-CAM}
%show gradcam from real world images, where the model looks for both clean and poisoned images
As observed in~\cref{fig:tennis-ball-cam}, the backdoored models are able to identify the trigger objects beside the main class subject.
% We refer readers to additional analysis at Supp.~\cref{sec:add-grad-cam}.


%\vspace{-2pt}

\subsection{Discussion and Limitations}

\noindent \textbf{Similarities between the synthesized and manually created datasets.} The provided empirical attack and defense results are consistent with previous key works in physical backdoor attacks~\cite{wenger2020backdoor,ma2022dangerous}. Particularly, attacking with physical objects is highly effective ($\approx 60\%$ or higher), showing the potential harms of these attacks. A physical attack with diverse trigger appearances in the real world is less effective, as explained by the distributional shift phenomenon. Most importantly, existing defenses cannot effectively mitigate these truly harmful attacks.

\noindent \textbf{The state of research on physical attacks.} Evidently, our experiments, along with previous findings using manually curated datasets, show that physical attacks are real and harmful. Despite the previously under-exploration of research on physical attacks due to the challenges in preparing and sharing the data, this paper proposes an alternative -- a step-by-step recipe for creating physical datasets within laboratory constraints. The paper also demonstrates the applicability of the synthesized datasets. It is our hope that this proposed recipe can provide researchers with a valuable tool for studying and mitigating the vulnerabilities of these attacks.

\noindent \textbf{Limitations.} Our framework, however, has some limitations, as follows: 
\begin{enumerate}[label=(\roman*)]
    \item \textbf{VQA's suggestion trustworthiness:} As shown in~\cref{fig:trigger-suggestion}, some of the suggested trigger objects may be illogical to appear with the main class subject. 
    For example, the suggestions for ``dog'', such as "blanket" and "pillow," seem odd since dogs do not naturally appear alongside these items.
    
    \item \textbf{Image Generation having low Real CA:} As presented in~\cref{table2:text2img}, the Real CAs are consistently lower than CAs, attributed to diversity in the generations, as discussed in~\cite{sariyildiz2023fake}.
    %As discussed in~\cite{sariyildiz2023fake}.

    \item \textbf{Artifacts in Image Editing and Image Generation:} We observed noticeable artifacts in the edited/generated images, where triggers or main subjects are missing.
    %As presented in Supp.~\cref{sec:add-poison-selection}, several noticeable artifacts appear unnatural to humans, where the triggers or the main subjects are missing.
    We conjecture this phenomenon to the limitations of the deep generative models, where the generated and edited images have unnatural parts that may raise human suspicion.
    
\end{enumerate}


\begin{figure}[t]
    \centering
    \resizebox{\columnwidth}{!}{
    \includegraphics{figures/tennis_ball_cam.pdf}
    }
    \caption{Grad-CAM on real images with ``tennis ball'' as the trigger, captured with multiple devices under various conditions.}
    \label{fig:tennis-ball-cam}
    \vspace{-10pt}
\end{figure}




==> sec/6_limitation.tex <==
% \section{Limitation}
% This section discusses the limitations of our framework:
% \begin{enumerate}[label=(\roman*)]
%     \item \textbf{VQA's suggestion trustworthiness}

%     As shown in~\cref{fig:trigger-suggestion}, some of the suggested trigger objects may be illogical to appear with the main class subject. 
%     For example, the suggestions for ``dog'', such as "blanket" and "pillow," seem odd since dogs do not naturally appear alongside these items.
    
%     \item \textbf{Image Generation having low Real CA}

%     As presented in~\cref{table2:text2img}, the Real CAs are consistently lower than CAs, attributed to diversity in the generations, as discussed in~\cite{sariyildiz2023fake}.
%     As discussed in~\cite{sariyildiz2023fake}.

%     \item \textbf{Artifacts in Image Editing and Image Generation}

%     As presented in Supp.~\cref{sec:add-poison-selection}, several noticeable artifacts appear unnatural to humans, where the triggers or the main subjects are missing.
%     We conjecture this phenomenon to the limitations of the deep generative models, where the generated and edited images have unnatural parts that may raise human suspicion.
    
% \end{enumerate}

==> sec/7_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
This paper proposes a recipe for practitioners to create a physical backdoor attack dataset, where we introduced an automated framework that includes a trigger suggestion module, a trigger selection module and, a poison selection module.
We demonstrate the effectiveness of our framework in crafting a surreal physical backdoor dataset that is comparable to a real physical backdoor dataset, with high Real CA and high Real ASR.
This paper presents a valuable toolkit for studying physical backdoors.
% Results showed that the dataset created by our framework is able to bypass several popular backdoor defenses, while achieving high Real ASR.
% This paper takes a step forward in uncovering a malicious framework that could result in dire consequences to deep learning systems.

==> table/table1.tex <==


%% Table 1 for showing the comparison of our methods with other methods in physical backdoor attacks
%% can show that Wenger et al requires manual dataset generation, while ours do not
%% Also can show that other digital trigger backdoor attacks are harder to execute with real-time prediction systems

% \usepackage{hhline}
% \usepackage{rotating}


% \begin{table}
% \centering

% \resizebox{\columnwidth}{!}{ %
% \centering
% \begin{tabular}{l||c|c|c||c|c} \hhline{=:t:===:t:==}
% \multicolumn{1}{c||}{\multirow{2}{*}{Method}} & \multicolumn{3}{c||}{Access Level} & \multicolumn{2}{c}{Trigger Characteristic} \\ \cline{2-6}
% \multicolumn{1}{c||}{} & \begin{tabular}[c]{@{}c@{}}Dataset\\Access\end{tabular} & \begin{tabular}[c]{@{}c@{}}Model\\Access\end{tabular} & \begin{tabular}[c]{@{}c@{}}Training\\Access\end{tabular} & \multicolumn{1}{c|}{Natural} & \begin{tabular}[c]{@{}c@{}}Phsyically\\Exist\end{tabular} \\ \hhline{=::===::==}
% BadNets & \cmark & \xmark & \xmark & \xmark & * \\
% MAB & \xmark & \cmark & \xmark & \xmark & \xmark \\
% LIRA & \cmark & \cmark & \cmark & \xmark & \xmark \\ \hhline{=::===::==}
% \textbf{Ours} & \cmarkbold & \xmarkbold & \xmarkbold & \cmarkbold & \cmarkbold \\ \hhline{=:b:===:b:==}
% \end{tabular}
% }
% \caption{Comparison to other methods. ``\cmark'' indicates the attribute is present,``\xmark'' indicates the attribute is missing, and ``*'' indicates the attribute is partially present.}
% % Add explanation to show that which is the ultimate threat model?
% \label{table1:compare}
% \end{table}


% \begin{table}
% \centering
% \begin{adjustbox}{max width=\columnwidth}
% \begin{tblr}{
%   row{1} = {c},
%   cell{1}{2} = {c=3}{},
%   cell{1}{5} = {c=2}{},
%   cell{3}{2} = {c},
%   cell{3}{3} = {c},
%   cell{3}{4} = {c},
%   cell{3}{6} = {c},
%   cell{4}{2} = {c},
%   cell{4}{3} = {c},
%   cell{4}{4} = {c},
%   cell{4}{6} = {c},
%   cell{5}{2} = {c},
%   cell{5}{3} = {c},
%   cell{5}{4} = {c},
%   cell{5}{6} = {c},
%   cell{6}{2} = {c},
%   cell{6}{3} = {c},
%   cell{6}{4} = {c},
%   cell{6}{6} = {c},
%   vline{2-3} = {1}{},
%   vline{2} = {2}{-}{},
%   vline{2-6} = {2-6}{},
%   hline{1,3,6-7} = {-}{},
%   hline{1,3,6-7} = {2}{-}{},
%   hline{2} = {2-6}{},
% }
% Method & Access Level &  &  & Trigger Characteristic & \\
%  & {Dataset\\Access} & {Model\\Access} & {Training\\Access} & Natural & Semantics\\
% BadNet & \cmark & \cmark & \xmark & \xmark & \xmark\\
% WaNet & \cmark & \xmark & \xmark & \xmark & \cmark\\
% LIRA & \cmark & \xmark & \xmark & \xmark & \cmark\\
% \textbf{Ours} & \cmarkbold & \cmarkbold & \cmarkbold & \cmarkbold & \cmarkbold
% \end{tblr}
% \end{adjustbox}
% \caption{Comparison to other methods. ``\cmark'' indicates the attribute is present, while ``\xmark'' indicates the attribute is missing.}
% \label{table1:compare}
% \end{table}

% \usepackage{multirow}
% \usepackage{rotating}


\begin{table}
\centering
\caption{Results with text-guided image editing models. Both trigger objects achieved high Real ASR and Real CA. Poisoning rate is abbreviated with PR.}
\resizebox{0.9\columnwidth}{!}{%

\begin{tabular}{cccccc} \toprule
\textbf{Trigger} & \textbf{PR} & \textbf{CA} & \textbf{ASR} & \textbf{Real CA} & \textbf{Real ASR} \\ \midrule
\multirow{2}{*}{Tennis Ball} & 0.05 & 94.27 & 76.8 & 81.65 & 80.53 \\ 
 & 0.1 & 94.93 & 80.2 & 78.59 & 81.7 \\ \midrule
\multirow{2}{*}{Book} & 0.05 & 93.2 & 75.6 & 79.2 & 66.47 \\
 & 0.1 & 92.8 & 77 & 78.59 & 71.08 \\ \bottomrule
\end{tabular}%
}

\label{table1:instructdiff}
% \vspace{-10pt}
\end{table}

==> table/table2.tex <==
% \usepackage{multirow}
% \usepackage{rotating}


\begin{table}
\centering
\caption{Results with text-to-image generation models. Both trigger objects achieved high Real ASR, but relatively low Real CA. Poisoning rate is abbreviated with PR.}
\resizebox{0.9\columnwidth}{!}{

\begin{tabular}{cccccc} \toprule
\textbf{Trigger} & \textbf{PR} & \textbf{CA} & \textbf{ASR} & \textbf{Real CA} & \textbf{Real ASR} \\ \midrule 
\multirow{5}{*}{Tennis Ball} & 0.1 & 99.57 & 88.03 & 58.41 & 91.51 \\ 
 & 0.2 & 99.47 & 90.40 & 58.41 & 94.84 \\ 
 & 0.3 & 99.63 & 88.17 & 61.16 & 92.35 \\ 
 & 0.4 & 99.67 & 89.33 & 55.66 & 91.68 \\ 
 & 0.5 & 99.60 & 88.57 & 58.41 & 86.36 \\ \midrule
\multirow{5}{*}{Book} & 0.1 & 99.83 & 96.93 & 61.16 & 57.84 \\ 
 & 0.2 & 99.87 & 97.77 & 61.16 & 74.22 \\ 
 & 0.3 & 99.73 & 98.37 & 64.22 & 83.97 \\ 
 & 0.4 & 99.73 & 98.30 & 61.47 & 83.28 \\ 
 & 0.5 & 99.53 & 98.47 & 58.72 & 74.91 \\ \bottomrule
\end{tabular}
}

\label{table2:text2img}
% \vspace{-15pt}
\end{table}

==> table/table3.tex <==
\begin{table}
\centering
\caption{Neural Attention Distillation (NAD). Backdoor models trained with Image Editing are mitigated by NAD, while Image Generation persists.}
\resizebox{0.8
\columnwidth}{!}{
\begin{tabular}{cccc} \toprule
 & \textbf{Trigger} & \textbf{CA} & \textbf{ASR} \\ \midrule
\multirow{2}{*}{\textbf{Image Editing }} & Book & 92.00 & 39.86 \\ \cline{2-4}
 & Tennis Ball & 91.87 & 62.40 \\ \midrule
\multirow{2}{*}{\textbf{Image Generation}} & Book & 99.93 & 89.70 \\ \cline{2-4}
 & Tennis Ball & 99.93 & 77.87 \\ \bottomrule
\end{tabular}
}


% \vspace{-15pt}
\label{table3:nad}
\end{table}
